Steady electric currents in magnetized QCD and their use for the equation of state

In this paper we study the emergence of steady electric currents in QCD as a response to a non-uniform magnetic background using lattice simulations with 2 + 1 quark flavors at the physical point, as well as leading-order chiral perturbation theory. Using these currents, we develop a novel method to determine the leading-order coefficient of the equation of state in a magnetic field expansion: the magnetic susceptibility of the QCD medium. We decompose the current expectation value into valence- and sea-quark contributions and demonstrate that the dominant contribution to the electric current is captured by the valence term alone, allowing for a comparably cheap determination of the susceptibility. Our continuum extrapolated lattice results for the equation of state confirm the findings of some of the existing studies in the literature, namely that the QCD medium behaves diamagnetically at low and paramagnetically at high temperatures.

==> introduction.tex <==
\begin{table}
  \begin{tabular}{lSSSSSS}
    \toprule
    \multirow{2}{*}{Dataset} &
      \multicolumn{2}{c}{A (\%)} &
      \multicolumn{2}{c}{B (\%)} &
      \multicolumn{2}{c}{C (\%)} \\
      & {O.B.R} & {A.R} & {O.B.R} & {A.R} & {O.B.R} & {A.R} \\
      \midrule
    D1 & 2.1 & 2.1 & 2.1 & 2.1 & 2.1 & 2.1 \\
    D2 & 11.6 & 11.6 & 11.6 & 11.6 & 11.6 & 11.6 \\
    D3 & 5.5 & 5.5 & 5.5 & 5.5 & 5.5 & 5.5 \\
    \bottomrule
  \end{tabular}
\end{table}

==> methods.tex <==
\section{Magnetic susceptibility}
%
In this section, we frist give a brief overview on how to compute the magnetic susceptibility from its thermodynamics definition via a current-current correlator (REFERENCE), and describe our new method to compute the magnetic susceptibility $\chi_m$ from the electric current density in a non-uniform background. In terms of the partition function, the magnetic susceptibility is defined as
%
\begin{equation}
\chi_m \equiv \pdv[2]{\log Z}{(eB)}\Bigg|_{eB=0} 
\end{equation}
%
where the second derivative is taken w.r.t. the renormalization group invariant $eB$. Using Maxwell's equations in a medium, the linear response coefficient $\chi_m$ to a $z$-oriented magnetic field $B(x)$ can be expressed in terms of the current as

The total magnetic field produced by a magnetized medium $\vec{B}/\mu_0=\vec{H}+\vec{M}$ is governed by Ampere's law
%
\begin{equation}
\frac{1}{\mu_0}\curl{\vec{B}} = \vec{J}_{f} + \vec{J}_m
\label{eq:ampere_law}
\end{equation}
%
where $\vec{J}_f = \curl \vec{H}$ is the free current flowing due to the presence of $\vec{H}$ and $\vec{J}_m = \curl \vec{M}$ is the magnetization current due to the response $\vec{M}$. The linear response to the field $\vec{B}$ is given by $\vec{M} = \chi_m \vec{H} \approx \chi_m \vec{B}$, where $\chi_m$ is the magnetic susceptibility. Replacing $\vec{M}$ in the equation of the current
%
\begin{equation}
\chi_m\curl\vec{B} = \vec{J}_m
\end{equation}

%
\begin{equation}
\chi_m\pdv{B(x)}{x} = J_m(x)
\label{eq:ampere_mu0=1}
\end{equation}
%
in units where the vacuum permeability $\mu_0 \equiv 1$. Since $\chi_m$ is a constant in space, we integrate Eq.~\eqref{eq:ampere_mu0=1} to get rid of the $x$-dependence on both sides
%
\begin{equation}
\chi_m = \dfrac{\int_{x_0}^{x_f} \dd x J_m(x)}{\int_{x_f}^{x_0} \dd x \partial B(x)/\partial x}
\label{eq:chi_m_int}
\end{equation}
%
where we chose $x_0 = -L_x/2$, $x_f = 0$. This corresponds to integrating the current and the magnetic field on the first half of the lattice. Even though different choices of the integration limits are also valid, the one we employed is particularly convenient, since it uses the largest number of independent data points in $x$. Notice that the choice $x_0=-L_x/2$, $x_f = L_x/2$ would lead to a vanishing result due to the antisymmetric profile of the current. To match the thermodynamic definition of $\chi_m$, we extrapolated the results from Eq.~\eqref{eq:chi_m_int} for $N_b=0$ using a quadradic function. The physical motivation for this ansatz is the symmetry of the partition function $Z(B) = Z(-B)$, which only allows for even powers of $B$ in the susceptibility. In Figure BLA, we show some examples of how this extrapolation is carried out


After the $B=0$ extrapolation, $\chi_m$ still contains an additive logarithmic divergence which has to be cancelled. Therefore, we follow (REFERENCE) and define the renormalized susceptibility as $\chi_m(T) = \chi^b_m(T)-\chi^b_m(0)$, for $\chi^b_m(T=0)$ contains the same divergent term, which is expected to be temperature independent.
%
\section{Electric current renormalization?}
wuciwcjhow
